Fine-grained Classification via Categorical Memory Networks

Motivated by the desire to exploit patterns shared across classes, we present a simple yet effective class-specific memory module for fine-grained feature learning. The memory module stores the prototypical feature representation for each category as a moving average. We hypothesize that the combination of similarities with respect to each category is itself a useful discriminative cue. To detect these similarities, we use attention as a querying mechanism. The attention scores with respect to each class prototype are used as weights to combine prototypes via weighted sum, producing a uniquely tailored response feature representation for a given input. The original and response features are combined to produce an augmented feature for classification. We integrate our class-specific memory module into a standard convolutional neural network, yielding a Categorical Memory Network. Our memory module significantly improves accuracy over baseline CNNs, achieving competitive accuracy with state-of-the-art methods on four benchmarks, including CUB-200-2011, Stanford Cars, FGVC Aircraft, and NABirds.

==> Fine-grained Classification via Categorical Memory Networks/dg_def.tex <==
% bold, vector,

\def\bb{{\bf b}}
\def\bc{{\bf c}}
\def\bd{{\bf d}}
\def\be{{\bf e}}
\def\bg{{\bf g}}
\def\bh{{\bf h}}
\def\bk{{\bf k}}
\def\bl{{\bf l}}
\def\bn{{\bf n}}
\def\bu{{\bf u}}
\def\bv{{\bf v}}
\def\bw{{\bf w}}
\def\bx{{\bf x}}
\def\by{{\bf y}}
\def\bz{{\bf z}}
\def\bm{{\bf m}}

\def\hatw{{\widehat w}}
\def\hatbw{{\widehat{\bf w}}}
\def\hatbz{{\widehat{\bf z}}}

\def\0{{\bf 0}}
\def\1{{\bf 1}}

\def\bA{{\bf A}}
\def\bB{{\bf B}}
\def\bD{{\bf D}}
\def\bE{{\bf E}}
\def\bH{{\bf H}}
\def\bI{{\bf I}}
\def\bM{{\bf M}}
\def\bP{{\bf P}}
\def\bS{{\bf S}}
\def\bZ{{\bf Z}}
\def\bR{{\bf R}}
\def\bK{{\bf K}}
\def\bX{{\bf X}}
\def\bY{{\bf Y}}
\def\bZ{{\bf Z}}



\def\bmu{\boldmath{\mu}}
\def\blambda{\boldmath{\lambda}}
\def\balpha{\mbox{{\boldmath $\alpha$}}}
\def\bpsi {\mbox{{\boldmath $\psi$}}}
\def\bPsi{\mbox{{\boldmath $\Psi$}}}
\def\bPi{\mbox{{\boldmath $\Pi$}}}
\def\bphi{\mbox{{\boldmath $\phi$}}}
\def\bPhi{\mbox{{\boldmath $\Phi$}}}
\def\bUpsilon{\mbox{{\boldmath $\Upsilon$}}}
\def\bLambda{\mbox{{\boldmath $\Lambda$}}}
\def\boldeta{\mbox{{\boldmath $\eta$}}}
\def\bOmega{\mbox{{\boldmath $\Omega$}}}
\def\bomega{\mbox{{\boldmath $\omega$}}}
\def\bzeta {\mbox{{\boldmath $\zeta$}}}
\def\bvarpi{\mbox{{\boldmath $\varpi$}}}
\def\btau {\boldsymbol{\tau}}
\def\bbeta{\mbox{{\boldmath $\beta$}}}
\def\bDelta{\mbox{{\boldmath $\Delta$}}}
\def\bdelta{\mbox{{\boldmath $\delta$}}}
\def\bxi{\mbox{{\boldmath $\xi$}}}


% \mathcal, function
\def\cA{{\mathcal A}}
\def\cC{{\mathcal C}}
\def\cD{{\mathcal D}}
\def\cF{{\mathcal F}}
\def\cG{{\mathcal G}}
\def\cH{{\mathcal H}}
\def\cK{{\mathcal K}}
\def\cL{{\mathcal L}}
\def\cN{{\mathcal N}}
\def\cM{{\mathcal M}}
\def\cS{{\mathcal S}}
\def\cR{{\mathcal R}}
\def\cT{{\mathcal T}}
\def\cU{{\mathcal U}}
\def\cW{{\mathcal W}}
\def\cX{{\mathcal X}}
\def\cY{{\mathcal Y}}

% \mathbb, domain
\def\mbA{{\mathbb A}}
\def\mbN{{\mathbb N}}
\def\mbR{{\mathbb R}}
\def\mbX{{\mathbb X}}
\def\mbZ{{\mathbb Z}}


\def\hatx{\widehat{\bx}}

% hat, tilde
\def\tx{\tilde{\x}}
\def\barx{\bar{\x}}
\def\tbPi{\mbox{{\boldmath $\tilde{\Pi}$}}}


% theorem
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{corollary}{Corollary }

%
\def\diag{\mbox{diag}}
\def\dist{\mbox{dist}}
\def\sgn{\mbox{sgn}}
\def\card{{\mbox{Card}}}

%
\def\etal{\emph{et al. }}
\def\ie{\emph{i.e.}}
\def\eg{\emph{e.g.}}
\def\etc{\emph{etc}}
\def\supp{\text{supp}}
\def\st{{\mathrm{s.t.}}}

%

\def\la{\langle}
\def\ra{\rangle}

%
\def\T{{\sf T}}
% \def\T{{\top}}




%%%%
\def\DIFFMAP{\mbox{{ ${\Phi_{\y_i,\y}}$}}}
\def\DIFFMAPCL{\mbox{{ ${\Phi^\mC_{\y_i,\y}}$}}}
\def\DIFFMAPCLK{\mbox{{ ${\Phi^{\mC^t}_{\y_i,\y}}$}}}
\def\DIFFMAPND{\mbox{{ ${\Phi^\mV_{\y_i,\y}}$}}}
\def\DIFFMAPcl{\mbox{{ ${\Phi^\mc_{\y_i,\y}}$}}}
\def\DIFFMAPCLKHAT{\mbox{{ ${\Phi^{\mU^t}_{\y_i,\y}}$}}}
\def\DIFFMAPGAMMA{\mbox{{ ${\Phi^{\Gamma_k}_{\y_i,\y}}$}}}
\def\DIFFMAPU{\mbox{{ ${\Phi^{\mU}_{\y_i,\y}}$}}}


%\def\gradim{{\nabla_{\eta}}}
% \def\gradim{{\nabla}}
\def\grad{{\nabla}}

%\def\xxxx{{\boldsymbol{\tau}_{\eta}}



\def\taux{\bm{\tau}_{\bf x}}
\def\kappax{\kappa_{\bf x}}
\def\kappaw{\kappa_{\bf w}}
\def\Lambdax{\Lambda_{\bf x}}
\def\Lambdaw{\Lambda_{\bf w}}
\def\bxi{\bm{\xi}}


%\def\dong{\textcolor{red}}%
\newcommand\mynote[1]{\textcolor{RedOrange}{#1}}
% \newcommand\mynote[1]{black}

